Hearing and Seeing Through CLIP: A Framework for Self-Supervised Sound Source Localization

Large-scale vision-language models demonstrate strong multimodal alignment and generalization across diverse tasks. Among them, CLIP stands out as one of the most successful approaches. In this work, we extend the application of CLIP to sound source localization, proposing a self-supervised method operates without explicit text input. We introduce a framework that maps audios into tokens compatible with CLIP's text encoder, producing audio-driven embeddings. These embeddings are used to generate sounding region masks, from which visual features are extracted and aligned with the audio embeddings through a contrastive audio-visual correspondence objective. Our findings show that alignment knowledge of pre-trained multimodal foundation model enables our method to generate more complete and compact localization for sounding objects. We further propose an LLM-guided extension that distills object-aware audio-visual scene understanding into the model during training to enhance alignment. Extensive experiments across five diverse tasks demonstrate that our method, in all variants, outperforms state-of-the-art approaches and achieves strong generalization in zero-shot settings.

==> Tables_black/comparison_openset_new.tex <==
\begin{table}
\vspace{-2mm}
\centering
\resizebox{1.0\linewidth}{!}{
\setlength{\tabcolsep}{3pt}
\begin{tabular}{clccccc}
\toprule
& \textbf{Method} & \textbf{cIoU} & \textbf{w/ Adap.} & \textbf{AUC} & \textbf{w/ Adap.} \\ 
    \midrule
    \multirow{14}{*}{\rotatebox[origin=c]{90}{\textbf{Heard}}}
    & LVS$_{\text{CVPR}21}$ & 28.90 & - & 36.20 & - \\
    & EZ-VSL$_{\text{ECCV}22}$ & 31.86 & - & 36.19 & - \\
    & EZ-VSL (w/ OGL)$_{\text{ECCV}22}$ & 37.25 & - & 38.97 & - \\
    & SLAVC$_{\text{NeurIPS}22}$ & 35.84 & - & - & - \\
    & SLAVC (w/ OGL)$_{\text{NeurIPS}22}$ & 38.22 & - & - & - \\
    & FNAC (w/ OGL)$_{\text{CVPR}23}$ & 39.54 & - & 39.83 & - \\
    & Alignment$_{\text{ICCV}23}$ & 38.31 & - & 39.05 & - \\
    & Alignment (w/ OGL)$_{\text{ICCV}23}$ & 41.85 & - & 40.93 & - \\
    \cline{2-6}
    & \textit{Baselines:} & & & & \\
    & \cellcolor{lightgray!25}\includegraphics[height=1em]{Figures/oracle.png}(\textbf{\textit{Oracle}}) CLIPSeg (w/ GT Text) & \cellcolor{lightgray!25}49.65 & \cellcolor{lightgray!25}64.86 & \cellcolor{lightgray!25}45.74 & \cellcolor{lightgray!25}55.78 \\
    & CLIPSeg (w/ WAV2CLIP Text) & 23.24 & 22.15 & 24.78 & 25.85 \\
    & CLIPSeg (w/ CLAP Text) & 19.93 & 23.99 & 29.56 & 26.54 \\
    & WAV2CLIP$_{\text{ICASSP}22}$ & 32.76 & - & 36.20 & - \\
    & AudioCLIP$_{\text{ICASSP}22}$ & 45.01 & - & 46.31 & - \\

    \cline{2-6}
    & \cellcolor{azure!10}\textit{\textbf{Ours}:} &  \cellcolor{azure!10} & \cellcolor{azure!10} & \cellcolor{azure!10} & \cellcolor{azure!10} \\
    & \cellcolor{azure!10}$\hookrightarrow$~w/ AV Alignment & \cellcolor{azure!10} 48.44 & \cellcolor{azure!10} 60.57 & \cellcolor{azure!10} 45.06 & \cellcolor{azure!10} 51.91 \\
    & \cellcolor{azure!10}$\hookrightarrow$~w/ AV + Caption Alignment & \cellcolor{azure!10} \textbf{50.27} & \cellcolor{azure!10} 63.18 & \cellcolor{azure!10} 45.16 & \cellcolor{azure!10} 53.15 \\
    
\bottomrule
\bottomrule
% \midrule
    \multirow{14}{*}{\rotatebox[origin=c]{90}{\textbf{Unheard}}}
& LVS$_{\text{CVPR}21}$ & 26.30 & - & 34.70 & - \\
    & EZ-VSL$_{\text{ECCV}22}$ & 32.66 & - & 36.72 & - \\
    & EZ-VSL (w/ OGL)$_{\text{ECCV}22}$ & 39.57 & - & 39.60 & - \\
    & SLAVC$_{\text{NeurIPS}22}$ & 36.50 & - & - & - \\
    & SLAVC (w/ OGL)$_{\text{NeurIPS}22}$ & 38.87 & - & - & - \\
    & FNAC (w/ OGL)$_{\text{CVPR}23}$ & 42.91 & - & 41.17 & - \\
    & Alignment$_{\text{ICCV}23}$ & 39.11 & - & 39.80 & - \\
    & Alignment (w/ OGL)$_{\text{ICCV}23}$ & 42.94 & - & 41.54 & - \\
    \cline{2-6}
    & \textit{Baselines:} & & & & \\
    & \cellcolor{lightgray!25}\includegraphics[height=1em]{Figures/oracle.png}(\textbf{\textit{Oracle}}) CLIPSeg (w/ GT Text) & \cellcolor{lightgray!25}49.13 & \cellcolor{lightgray!25}65.59 & \cellcolor{lightgray!25}44.77 & \cellcolor{lightgray!25}55.39 \\
    & CLIPSeg (w/ WAV2CLIP Text) & 26.25 & 24.78 & 27.03 & 28.48 \\
    & CLIPSeg (w/ CLAP Text) & 23.65 & 26.33 & 32.14 & 28.92 \\
    & WAV2CLIP$_{\text{ICASSP}22}$ & 34.80 & - & 37.72 & - \\
    & AudioCLIP$_{\text{ICASSP}22}$ & 43.30 & - & 46.14 & - \\
    \cline{2-6}
    & \cellcolor{azure!10}\textit{\textbf{Ours}:} &  \cellcolor{azure!10} & \cellcolor{azure!10} & \cellcolor{azure!10} & \cellcolor{azure!10} \\
    & \cellcolor{azure!10} $\hookrightarrow$~w/ AV Alignment & \cellcolor{azure!10} 41.98 & \cellcolor{azure!10} 55.88 & \cellcolor{azure!10} 41.55 & \cellcolor{azure!10} 49.36 \\
    & \cellcolor{azure!10} $\hookrightarrow$~w/ AV +  Caption Alignment  & \cellcolor{azure!10} \underline{45.71} & \cellcolor{azure!10} 59.73 & \cellcolor{azure!10} \underline{43.58} & \cellcolor{azure!10} 51.25 \\



\bottomrule
    
    \end{tabular}}
    \caption{\textbf{Comparison results on open-set audio-visual localization.} All the experiments are trained and tested on the same splits of prior works. Note that prior works did not release their models trained on this dataset; thus, adaptive scores are unavailable, and all numbers are reported from their papers.}
    {
    \label{tab:exp_openset_first}}
    \vspace{-4mm}

\end{table}

==> def_custom.tex <==
% % % % % %
% % For IEEE journal version formatting
\usepackage{xspace}
\makeatletter
\def\onedot{\ifx\@let@token.\else.\null\fi\xspace}
\makeatother
% % % % % % %


\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother

\def\eg{\textit{e.g}\onedot} \def\Eg{{E.g}\onedot}
\def\ie{\textit{i.e}\onedot} \def\Ie{{I.e}\onedot}
\def\cf{\textit{c.f}\onedot} \def\Cf{{C.f}\onedot}
\def\etc{\textit{etc}\onedot} \def\vs{{vs}\onedot}
\def\wrt{\textit{w.r.t}\onedot} \def\dof{d.o.f\onedot}
\def\etal{\textit{et al}\onedot}



\newcommand{\Tref}[1]{Table~\ref{#1}}
\newcommand{\Eref}[1]{Eq.~(\ref{#1})}
\newcommand{\Fref}[1]{Figure~\ref{#1}}
\newcommand{\FCref}[1]{Chapter.~\ref{#1}}
% \newcommand{\Cref}[1]{Chap.~\ref{#1}}
\newcommand{\Sref}[1]{Section~\ref{#1}}
\newcommand{\Aref}[1]{Alg.~\ref{#1}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\matL}{\mathbf{Z}}
\newcommand{\matS}{\mathbf{E}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\Z}{\mathbf{Z}}

\newcommand{\CovX}{\mathbf{\Phi}}
\newcommand{\CovS}{\mathbf{\Gamma}}

\newcommand{\D}{\mathbf{D}}
\newcommand{\singularmat}{\Sigma}

\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\newcommand{\newpara}[1]{\vspace{6pt}\noindent\textbf{#1}}

\def\Vec#1{\mbox{\boldmath $#1$}}
\newcommand{\mO}{\mathbf{O}}
\newcommand{\mc}{\mathbf{c}}

\newcommand{\paragrp}[1]{\vspace{1mm}\noindent\textbf{#1}\,\,\,}


\newcommand{\arda}[1]{\textcolor{blue}{#1}}
\newcommand{\soo}[1]{\textcolor{gray}{Sooyoung: {#1}}}

\definecolor{golden}{RGB}{255, 215, 0}
\definecolor{softgold}{RGB}{238, 180, 34}
\definecolor{lightgold}{RGB}{250, 240, 200}
\definecolor{lightgold_v2}{RGB}{255, 243, 191}
\definecolor{azure}{rgb}{0.0, 0.5, 1.0}
\definecolor{PastelGreen}{rgb}{0.13, 0.55, 0.13}


